Bias-Variance Games

Firms engaged in electronic commerce increasingly rely on predictive analytics via machine-learning algorithms to drive a wide array of managerial decisions. The tuning of many standard machine learning algorithms can be understood as trading off bias (i.e., accuracy) with variance (i.e., precision) in the algorithm's predictions. The goal of this paper is to understand how competition between firms affects their strategic choice of such algorithms. To this end, we model the interaction of two firms choosing learning algorithms as a game and analyze its equilibria. Absent competition, players care only about the magnitude of predictive error and not its source. In contrast, our main result is that with competition, players prefer to incur error due to variance rather than due to bias, even at the cost of higher total error. In addition, we show that competition can have counterintuitive implications -- for example, reducing the error incurred by a firm's algorithm can be harmful to that firm -- but we provide conditions under which such phenomena do not occur. In addition to our theoretical analysis, we also validate our insights by applying our metrics to several publicly available datasets.

==> MSmath.tex <==
\newcommand{\setsize}[1]{{\left|#1\right|}}

\newcommand{\floor}[1]{
{\lfloor {#1} \rfloor}
}
\newcommand{\bigfloor}[1]{
{\left\lfloor {#1} \right\rfloor}
}



%\DeclareMathOperator{\argmax}{argmax}
%\DeclareMathOperator{\argmin}{argmin}

\newcommand{\super}[1]{^{(#1)}}

\newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\tinteval}[1]{\left[#1\right]}
\newcommand{\distcond}[2]{\left.#1\vphantom{\big|}\right|_{#2}}
\newcommand{\evalat}[2]{\left.#1\vphantom{\big|}\right|_{#2}}


%
% probability stuff.
%
\newcommand{\given}{\,\mid\,}

% resizing brackets 
\newcommand{\prob}[2][]{\text{\bf Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\expect}[2][]{\text{\bf E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\var}[2][]{\text{\bf Var}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}


% brackets configured with \tparen
\newcommand{\tparen}{\big}
\newcommand{\tprob}[2][]{\text{\bf Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\tparen[{\def\given{\tparen|}#2}\tparen]}
\newcommand{\texpect}[2][]{\text{\bf E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\tparen[{\def\given{\tparen|}#2}\tparen]}


% brackets do not resize.
\newcommand{\sprob}[2][]{\text{\bf Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}[#2]}
\newcommand{\sexpect}[2][]{\text{\bf E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}[#2]}






\newcommand{\suchthat}{\,:\,}


\newcommand{\partialx}[2][]{{\tfrac{\partial #1}{\partial #2}}}
\newcommand{\nicepartialx}[2][]{{\nicefrac{\partial #1}{\partial #2}}}
\newcommand{\dd}{{\mathrm d}}
\newcommand{\ddx}[2][]{{\tfrac{\dd #1}{\dd #2}}}
\newcommand{\niceddx}[2][]{{\nicefrac{\dd #1}{\dd #2}}}
\newcommand{\grad}{\nabla}

\newcommand{\symdiff}{\triangle}



==> aj_welfare.tex <==
\section{Aleck scratch}



==> general-framework.tex <==


\section{Overview of the General Framework}\label{sec:general-framework}
We begin by sketching a general framework of statistical decision theory, which is our point of departure.
For more details and references see \cite{friedman2001elements}.


Suppose there is some function $f:\R^n\mapsto\R$, and that $y=f(x)+\eps$ for a random variable $\eps$ with mean 0 and variance $\sigma^2$. Assume also that there is some prior distribution $\pi$ over $x$. A typical example is that $f$ is linear and 
$\eps$ is normally distributed, namely
$$y=f(x_1,\ldots,x_n)+\eps = \beta_0+\sum \beta_i x_i + \eps,$$
where the $\beta_i$'s are some fixed but unknown parameters.

A learning algorithm takes training data $D=\{(x^1,y^1),\ldots,(x^m,y^m)\}$ as input, and produces an estimator $\hat f$ as output. Given a new point $x$, the estimator $\hat f$ predicts that the corresponding value of $y$ is $\hat f(x;D)$.

Define the {\em loss} of a learning algorithm at point $(x,y)$ as
$$L(\hat f, x) = \left(\hat f(x;D) - y\right)^2.$$
Note that the loss is random---it depends on both the randomness in $D$ and the randomness inherent in $\eps$.

The {\em risk} function of a learning algorithm at the point $(x,y)$ is 
$$R(\hat f, x) = \E[L(\hat f, x)],$$
where the expectation is taken over both
the randomness in $D$ that produced $\hat f$ and the randomness in $\eps$ (but note that $x$ is fixed).

A well-known result is that when the loss is defined as above (squared-loss), then the risk can be decomposed into bias and variance:
$$R(\hat f, x) = \left(\E_D[\hat f(x;D)]-f(x)\right)^2 + \mathrm{Var}[\hat f(x;D)] + \sigma^2,$$
where $\E[\hat f(x;D)]-\E[f(x)]=\mathrm{Bias}_D[\hat f(x;D)]$ 
\yf{$f(x)$ instead of $\expect{f(x)}$?} 
is the {\em bias} of the estimator at $x$, the second term is the {\em variance} of the estimator (computed with respect to the randomness of $D$) at $x$, and the third term is the {\em irreducible error}. 

Ideally, we would like our learning algorithm to have minimal risk for all $x$'s. However, this is generally not possible. Instead, one way of identifying a good algorithm is to find one that minimizes  the {\em Bayes risk} $$R_B(\hat f) = E_{x}[R(\hat f, x)].$$
The Bayes risk can be decomposed into expected bias and expected variance:
$$R_B(\hat f) = \E_x\left[\mathrm{Bias}_D[\hat f(x;D)]^2\right] + \E_x\left[\mathrm{Var}[\hat f(x;D)]\right] + \sigma^2.$$


Now, in general we may not know the distribution over $x$'s, and in this case a common approach is to consider the {\em empirical risk}
$$R_{\mathrm{emp}}(\hat f) = \frac{1}{m}\sum_{i=1}^m  L(\hat f(x^i;D), y^i)$$
of an estimator. Minimizing the empirical risk is not helpful, since one could always choose $\hat f$ for which $\hat f(x;D) = y$ when $(x,y)\in D$, and $\hat f(x;D) = 0$ otherwise. Common ways to get around this problem are (i) to limit the class of functions from which $\hat f$ is chosen, and (ii) to find an estimator that minimizes the {\em regularized} empirical risk
$$R_{\mathrm{emp}}(\hat f) + \lambda J(\hat f).$$
Here, $\lambda\in \R_+$ is a {\em regularization parameter} and $J$ is some penalty function. For example, in ridge regression, the goal is to find a linear estimator $\hat f(x;D) = \hat \beta_0 + \sum_{i=1}^n \hat \beta_i x_i$ such that $R_{\mathrm{emp}}(\hat f) + \lambda\sum_{i=1}^n {\hat\beta_i}^2$ is minimal.

In regularized empirical risk minimization, there are various ways to choose the regularization parameter $\lambda$. The goal is to choose $\lambda$ so that the Bayes risk of the resulting estimator is minimal. Typically, modifying $\lambda$ affects the bias and variance of an estimator. For example, in ridge regression, increasing $\lambda$ decreases the {\em expected} variance and increases the {\em expected} bias of the chosen estimator. At the optimal $\lambda$, the tradeoff between expected bias and expected variance of the chosen estimator is such that its Bayes risk is minimal.

The following subtlety is important for our paper. Even though increasing $\lambda$ decreases expected variance and increases expected bias, it may have different effects on the biases and variances at specific points $x$.

==> glossary.tex <==
\begin{figure}[t] \small
  \begin{center}
  \begin{minipage}{.95\textwidth}
    \ifaer
    \medskip
    \else
    \begin{center}
      Machine learning terminology:
    \end{center}
    \fi
    \begin{description}\setlength{\parskip}{0in}\setlength{\itemsep}{0in}
    \item[features:] observable quantities of a data point.
    \item[label:] quantity to be predicted for each data point.
    \item[hypothesis:] a function that maps the features of a data
      point to a {\bf prediction}.
    \item[hypothesis set:] a set of allowable hypotheses that the
      algorithm could select.
    \item[training set:] the data that the algorithm is trained on;
      contains features and a label for each data point.
    \item[algorithm:] a procedure that considers the data in the
      training set and chooses a hypothesis.      
    \item[test set:] the data that the hypothesis of the algorithm is
      evaluated against; for each data point, the prediction of the hypothesis is
      compared to the true label.
      \item[mean squared error:] a measurement of error of a
        hypothesis as the squared difference between the true and
        predicted labels averaged over a data set.
    \item[accuracy; bias:] quantification of how far the average
      prediction is from the true label. \\ (Related terms: {\bf under-fitting}, {\bf representation error}.) 
    \item[precision; variance:] quantification of the concentration of predictions around their average. \\ (Related terms: {\bf over-fitting}, {\bf generalization error}.) 
%    \item[regularization:] a method of penalizing complex hypotheses that decreases variance and increases bias.
    \item[regularization:] an algorithmic method for penalizing complex hypotheses to avoid over-fitting.
    \end{description}
    \ifaer\else
    \begin{center}
      Game theory terminology:
    \end{center}
    \begin{description}\setlength{\parskip}{0in}\setlength{\itemsep}{0in}
    \item[action:] choice of a player in a game.
    \item[action space:] set of possible actions a player can take.
    \item[payoff:] the benefit that a player in a game receives.
    \item[best response:] an action that maximizes a player's payoff
      given the actions of the other players.
    \item[dominant strategy:] an action that is a best response to any combinations of actions of the other players.
    \item[Nash equilibrium:] actions for each player that are best responses to one another.
    \item[individual rationality:] each player in a game has an      
      action that guarantees non-negative payoff.
    \end{description}
    \fi
  \end{minipage}
  \end{center}
  \caption{%
    \label{fig:terminology-guide}
    Guide to \ifaer machine learning \fi terminology.
  }
\end{figure}


==> organization.tex <==
\section{Overview and Organization of Results}
\Cref{sec:general-framework} provides an overview of the general framework of statistical decision theory. For clarity, we distinguish between two stages of this framework within which we perform analysis:
\begin{enumerate}
    \item The {\em ex ante} stage: At this stage the analyst has obtained a dataset, and has to choose an estimator $\hat f$. A running example we use is that they choose a regularization parameter $\lambda$ and the corresponding ridge estimator  $\hat f_\lambda$.
    \item The {\em interim} stage: At this stage a new feature vector $x$ is realized, and the analyst uses the chosen estimator to predict the label of $x$. Running assumptions for our theoretical analyses here are that predictions are normally distributed and have total error 1.
\end{enumerate}

In practice, we are interested in what happens at the ex ante stage, as this is where we have to make a choice. However, in terms of analysis, it is often convenient to study the interim stage \citep[see, e.g.,][]{friedman2001elements}. For example, the bias-variance decomposition is often stated for the interim stage. In this paper, we have results for both stages, as listed below.

One possible organization of the paper would be to start with 2(a), then do the interim stuff 1(a)-1(g), and finally return to ex ante 2(b)-2(h). Some of the justifications of assumptions would naturally be pushed to the Appendix. I'm not sure about the optimal ordering of 1(d) and 1(g).

\begin{enumerate}
\item \textbf{Results pertaining to interim stage}
\begin{enumerate}
    \item \Cref{sec:prelim} contains the model and preliminaries for the interim stage. It includes our first assumption, namely, the form of players' utility functions.
    \item \Cref{sec:no-tradeoff} gives counter-intuitive examples about what can happen in the bias-variance game: namely, reducing variance or bias (all else fixed) can be harmful. There are also results about reducing bias being beneficial for convex and normal distributions of prediction error.
    \item \Cref{sec:main-analysis} is our main result: when distributions are normal and bias-variance tradeoff is 1, lowering bias (and increasing variance) is ex post dominant.
    \item \Cref{sec:non-constant-tradeoff} shows that the main insight persists when bias-variance tradeoff is not fixed. This uses an assumption on the continuity and differentiability of the tradeoff.
    \item \Cref{sec:normal-motivation} and \Cref{app:normal-motivation} have formal motivation for the normality assumption (in the context of ridge regression).
    \item \Cref{fig:ridge-normal} in \Cref{sec:empirical} has an empirical ``demonstration'' of the normality assumption.
    \item \Cref{sec:numerical} has numerical results for other distributions and payoffs. NEED TO ADD: Yiding's new simulations for different bias-variance tradeoffs.
\end{enumerate}

\item \textbf{Results pertaining to ex ante stage}
\begin{enumerate}
    \item \Cref{sec:general-framework} provides an overview of the general framework, including both stages.
    \item \Cref{sec:empirical} demonstrates the preference for lower bias and higher variance empirically (in the context of ridge regression and on a particular dataset).
    \item \Cref{sec:non-constant-tradeoff-general-framework} has our main theoretical result on preference for lower $\lambda$ in the ex ante stage. It is based on assumptions numbered A1-A5.
    \item Assumption A1 is a normality assumption, same as in the interim stage.
    \item Assumption A2 is that our interim results hold for general bias-variance tradeoffs, a fact demonstrated numerically in 1(g).
    \item Assumption A3 is that increasing $\lambda$ increases bias and decreases variance for every feature vector $x$. \Cref{apx:multidimensional-ridge} analyzes ridge regression in a multidimensional model, where we can show that A3 holds.
    \item Assumption A4 is a continuity and differentiability assumption, similar to the one made in 1(d).
    \item Assumption A5 is that two particular random variables are negatively correlated. \Cref{apx:one-dimensional-ridge} analyzes ridge regression in a one-dimensional model, where we can show that assumption A5 holds.
\end{enumerate}
\end{enumerate}

==> prelim.tex <==
\section{Model and Preliminaries}
\label{sec:prelim}

In general, a learning algorithm $A$ takes training set
$D=\{(x_1,f(x_1)),\ldots,(x_m,f(x_m))\}$ as input, and outputs a
hypothesis $\hat f$ that maps features of new data points to a
predicted label.  Given a new point $(x,f(x))$, an algorithm's prediction
of the true label $f(x)$ is denoted $\hat f(x)$. In this paper, we will abstract
away from the algorithm itself, and will only be concerned with the
algorithm's error in prediction, $|f(x) - \hat f(x)|$, viewed as a
distribution over $\R$. The randomness in this distribution arises
both from the algorithm $A$ itself and from the inherent randomness of the
dataset and the choice of $x$. The best prediction is thus one with predictive error
of~0. 

We will focus on a standard measure of total error, namely, 
mean squared error. Thus, if the predictive error of an algorithm is a number $|a|$, then the squared
error is $a^2$.

%Furthermore, since we will suppose that the prediction task $x$ is fixed, we will assume without loss of generality that $f(x)=0$.

This paper is concerned with players' choices of algorithms. In our abstraction we will thus let each player choose a distribution over errors, from some class of distributions, as follows.  Fix a random variable $Z$ with mean 0 and standard deviation 1. A common choice for $Z$ will be normal, a choice we motivate in \Cref{sec:normal-motivation}, but we can
also consider uniform, triangle, Laplace, and other distributions. Players will then choose a distribution from a class
made up of shifts and spreads of $Z$. A typical example will be the class 
$$\X_Z=\left\{\sigma Z+\mu:\mu^2+\sigma^2\geq 1\right\},$$
the set of distributions whose bias squared plus variance is at least 1 (which means their total squared error
is at least 1). Each element of this class yields a different distribution over predictive error, and
represents a different algorithm whose error has the corresponding distribution.

Some discussion of this modelling assumption is warranted. The class of distributions $\X_Z$ represents the error distributions
of {\em all} algorithms available to a player. In particular, this precludes the possibility that a player chooses an algorithm, 
observes the realized prediction, and then uses some alteration of that prediction. For a concrete example of what this implies, consider the distribution $X$ with bias $\mu=1$ and variance $\sigma^2=0$, and observe that $X\in\X_Z$ above. Then our assumption precludes the possibility that the player takes the realization of $X$ and subtracts 1 from it. Although this results in a prediction with 0 total error, 
and is thus a perfect predictor, our view is that if a perfect predictor were available to the player then it would be included
in the set $\X_Z$.


\subsection{One player}\label{sec:one-player} As a benchmark, consider a setting in which there is only one player, and suppose that she chooses an error distribution $X$.
On realization $a$ (that is, a prediction with predictive error $a$), let the player's utility be $u(a) = 1-a^2$: a benefit of 1 minus her squared error.
This utility function captures the idea that the player obtains positive utility from making a perfect prediction (the benefit of 1),
but that this utility decreases with the squared error (the loss of $a^2$). In the box subscription company example from the
introduction, the benefit represents future profits from a particular customer, whereas the loss accounts for the
lack of customer retention in case of inaccurate taste predictions. Note that the total utility $1-a^2$ could be negative;
in the example this would represent a firm's failure to recoup the costs of an initial loss leader or promotion.
We focus on this utility function for our theoretical analysis, but in \Cref{sec:numerical} 
we argue that our results are robust to other specifications of the utility
function, and in particular to ones where the chance of a negative payoff is negligible.

Given the utility function $u(a) = 1-a^2$, a player's expected utility from $X$ is 
$u(X)=\expect{u(X)} = 1 - \expect{X^2}$. The following is a simple observation:

\begin{claim}\label{claim:util}
If $X=\sigma Z+\mu$, where $Z$ is a random variable with mean 0 and variance 1, then $u(X) = 1-\mu^2-\sigma^2$.
\end{claim}

\ifMS
\proof{Proof.}
\else\begin{proof}
\fi
$X$ is a random variable with variance $\sigma^2$ and expected value $\mu$. Since $\sigma^2=\var{X} = \expect{X^2}-\expect{X}^2 =\expect{X^2}-\mu^2$,
it follows that $\expect{X^2} = \sigma^2+\mu^2$. Thus, $u(X) = 1-\expect{X^2} = 1-\mu^2-\sigma^2$.
% The random variable $X$ has variance $\sigma^2$ 
% and expected value $\mu$. 
% Since $\sigma^2=\mathrm{Var}\left[X\right] = \mathrm{E}\left[X^2\right]-\mathrm{E}\left[X\right]^2 =\mathrm{E}\left[X^2\right]-\mu^2$,
% it follows that $\mathrm{E}\left[X^2\right]= \sigma^2+\mu^2$. Thus, $u(X) = 1-\mathrm{E}\left[X^2\right] = 1-\mu^2-\sigma^2$.
\ifMS
\Halmos
\endproof
\else \end{proof}
\fi

% \begin{proof} $X$ is a random variable with variance $\sigma^2$ and expected value $\mu$. Since $\sigma^2=\var{X} = \expect{X^2}-\expect{X}^2 =\expect{X^2}-\mu^2$,
% it follows that $\expect{X^2} = \sigma^2+\mu^2$. Thus, $u(X) = 1-\expect{X^2} = 1-\mu^2-\sigma^2$.
% \end{proof}

This observation implies three corollaries, formalized below. First, for fixed bias, the
player prefers minimal variance. Similarly, for fixed variance, the
player prefers minimal bias.  Finally, the player is indifferent
between distributions that have the same bias squared plus variance. Although these corollaries are 
straightforward, in \ifitcssubm\Cref{appx:no-tradeoff} \else Section~\ref{sec:all-else-fixed} \fi we will show that, without further assumptions, none of them 
hold in the competitive setting.


\begin{corollary}
For any $\mu$, if $\sigma<\sigma'$, then the player prefers $X=(\sigma Z+\mu)$ to $X'=(\sigma' Z+\mu)$.
\end{corollary}

\begin{corollary}
For any $\sigma$, if $\mu^2<\nu^2$, then the player prefers $X=(\sigma Z+\mu)$ to $X'=(\sigma Z+\nu)$.
\end{corollary}

\begin{corollary}
If $X=\sigma Z +\mu$, $X'=\tau Z + \nu$, and 
$\mu^2+\sigma^2 = \nu^2+\tau^2$, 
then the player is indifferent between $X$ and $X'$.
\end{corollary}

\paragraph{Individual rationality.}
An additional definition that will be useful is that of individual
rationality. Intuitively, a distribution is individually
rational if a player derives non-negative utility from
choosing it. Formally:
\begin{definition}
A distribution $X$ satisfies {\em individual rationality (IR)} if
$u(X)\geq 0$.
\end{definition}
A simple observation that follows from \Cref{claim:util}
is that $X=\sigma Z+\mu$ is IR if and only if $\mu^2+\sigma^2\leq 1$.

\subsection{Two players}
Recall that our goal is to analyze the effect of competition on firms' choices of learning algorithms.
As described in the introduction, we will model this as a game, and we call this game the {\em Bias-Variance Game}.
In this game, each of two players simultaneously chooses an error distribution. Prediction errors are realized, and the
player with lower prediction error, say $a_i$, obtains utility $1-a_i^2$, just like the one-player case. The player
with higher prediction error obtains utility 0. 

This specification of utilities, as well as variants that we discuss in \Cref{sec:numerical}, capture the
main competitive force we wish to analyze: the desire of a player both to minimize error (this is the $-a_i^2$ term), and to obtain lower
error than her competitor (this is the benefit of 1 from winning).

In our notation, when discussing player $i\in\{1,2\}$, we will denote by $j=3-i$ the identity of the other player. 
A formal description of the game follows:
\begin{definition}[The Bias-Variance Game]\label{BVG} Given two classes of distributions, $\X_1$ and $\X_2$, 
the two player bias-variance game proceeds as follows:
\begin{enumerate}
\item Each player $k \in \{1,2\}$ simultaneously chooses a distribution $X_k$ from $\X_k$.
\item Each $X_k$ is realized as some $a_k$.
\item Each player $i$ obtains utility $u_i(a_i, a_j) = (1 - a_i^2)\cdot {\bf 1}\{a_i < a_j\}$. That is,
the player $i \in \argmin_k a_k$ wins and obtains utility $u_{i}(a_{i},a_{j})=1-a_{i}^2$; the other player, $j$, loses and obtains utility  $u_{j}(a_{j},a_{i})=0$. 
\end{enumerate}
\end{definition}


In our theoretical analysis we will primarily consider bias-variance games where $\X_1 = \X_2 =
\X$ is a family of distributions in which the error of every $X \in \X$ is normalized
to $\mu^2 + \sigma^2 = 1$. In our numerical analysis in \Cref{sec:numerical} we relax this restriction.

\paragraph{Individual rationality.}
As in the one-player benchmark, we will be interested in player choices that are individually rational. A straightforward result is that
individual rationality of the one-player setting implies individual
rationality of the two-player setting, as the following proposition demonstrates:

\begin{proposition}
Bias-variance games with distributions $X \in \X$ satisfying $\mu^2 +
\sigma^2 \leq 1$ are individually rational: namely, expected payoffs in
the game are non-negative.
\end{proposition}

\ifMS \proof{Proof.}
\else\begin{proof}\fi
In the one-player setting player $i$'s expected payoff with realization $a_i
\sim X_i$ is $\expect{1-a_i^2} \geq 0$ which satisfies individual rationality.  Consider the two-player
game where the other player $j = 3-i$ has realization
$a_j$.  When the other player's realization is $|a_{j}| \leq 1$, the payoff
of player $i$ is non-negative for all $a_i$: for $|a_i| \leq |a_{j}|
\leq 1$ player $i$ wins and has non-negative payoff $1-a_i^2$ and for
$|a_i| > |a_{j}|$ then player $i$ loses and has payoff 0.  When the
other player's realization is $|a_{j}| > 1$, then player $i$'s
distribution of payoffs in the two player game dominates his
distribution of payoffs in the one-player setting (when player $i$ loses, instead of a negative payoff her payoff is zero).  As the latter
setting had non-negative expectation, so does the former.
\ifMS\Halmos\endproof
\else \end{proof}\fi

\paragraph{Solution concepts.} \ifaer We will consider various solution concepts.
\else
When there is a single player, the concept of optimality is
straightforward. When there are more players, however, different actions may be
better depending on the actions of other players.   ``Solutions'' to
games thus consist of finding strategies of players that satisfy
different notions of equilibrium. \fi For our main theoretical result on
the preference of variance over bias we will utilize a very strong
notion, namely that of ex post dominant strategies.  A strategy is ex
post dominant for player $i$ if it yields that player the highest
utility regardless of the {\em realized} prediction of the opponent.
\begin{definition} A strategy $X_i\in\X_i$ is {\em ex post dominant} for player $i$ if for all $X_i'\in\X_i$ and all realizations
$a_j$ of player $j$ it holds that $u_i(X_i,a_j)\geq u_i(X_i',a_j)$.
\end{definition}


For our numerical and empirical results we will consider two weaker
notions. The first, dominant strategies, requires that a strategy be
optimal against any strategy of the opponent, but not necessarily
against any realization of that strategy:
\begin{definition}
  A strategy $X_i\in\X_i$ is {\em dominant} for player $i$ if for all
  $X_i'\in\X_i$ and all $X_j\in\X_j$ it holds that $u_i(X_i,X_j)\geq
  u_i(X_i',X_j)$. If the inequality is strict for all $X_i'\neq X_i$, then $X_i$ is {\em strictly dominant}.
\end{definition}

The second, pure Nash equilibrium, does not require that a strategy be
optimal against any strategy of the opponent, but only against that
player's own Nash equilibrium strategy:
\begin{definition} A strategy profile $(X_1,X_2)$ is a {\em pure Nash equilibrium}
if for each player $i$ and strategy $X_i'\in\X_i$ it holds that $u_i(X_i,X_j)\geq u_i(X_i',X_j)$.
\end{definition}

Observe that if $X_i$ is ex post dominant, then it is also dominant. Furthermore, if $X_1$ and $X_2$ are dominant for players $1$ and $2$, respectively, then $(X_1,X_2)$ is a pure Nash equilibrium. Finally, if $X_1$ and $X_2$ are strictly dominant then $(X_1,X_2)$ is the {\em unique} Nash equilibrium.

%\begin{theorem}
%Fix a pair $(Z_1,Z_2)$, and let $\X_1=\{\sigma Z_1+\mu:(\mu,\sigma)\in C_1\}$ and $\X_2=\{\sigma Z_2+\mu:(\mu,\sigma)\in C_2\}$,
%where $C_1$ and $C_2$ are compact, convex subsets of $\R^2$. Then the game has a PNE.
%\end{theorem}






==> summary.tex <==

\begin{center}
    \begin{Large}
    Bias-Variance Games: Summary
    \end{Large}
\end{center}
%\author{Feng \and Gradwohl \and Hartline \and Johnsen}

\begin{center}
Yiding Feng ~~~~ Ronen Gradwohl ~~~~ Jason Hartline ~~~~ Aleck Johnsen ~~~~ Denis Nekipelov
\end{center}
%\date{}							% Activate to display a given date or no date


Firms engaged in electronic commerce increasingly rely on machine
learning algorithms to drive a wide array of managerial decisions.
The goal of this paper is to understand how competition between firms
affects their strategic choice of such algorithms. We model the
interaction of two firms choosing learning algorithms as a game, and
analyze its equilibria in terms of the resolution of the bias-variance
tradeoffs faced by the players.  We show that competition can lead to
strange phenomena---for example, reducing the error incurred by a
firm's algorithm can be harmful to that firm---and provide conditions
under which such phenomena do not occur. We also show that players
prefer to incur error due to variance than due to bias. Much of our
analysis is theoretical, but we also show that our insights persist
empirically in several publicly-available data sets.

In most of the paper we abstract away from the details of specific algorithms, and instead model an algorithm as a distribution
over predictions. Thus, players' sets of actions in the game are a class parameterized by a distribution, with elements ranging over biases and variances. 
%Thus, players' sets of actions in the game consist of several distributions with different biases and variances. 
A canonical example is the set of normal distributions with different means and standard deviations. 

For our first set of results, we show that there are classes of
distributions and opponent's choices for which a player prefers to
choose a distribution with higher bias (resp., variance) holding
variance (resp., bias) fixed, contrary to their optimal choices absent
competition. Next, our main theoretical result is that if a player's
action set consists of normal distributions, then this preference for
lower bias holds even if the variance is not fixed. 
That is, for two
normal distributions with the same total error, the player prefers the
one with lower bias (and higher variance) regardless of the
realization of the opponent's choice. Formally in the game we analyze,
each player $i$ chooses a bias $\mu_i \in [0,1]$ and receives a draw $a_i$ from $\N(\mu_i,\sqrt{1-\mu_i^2})$; the player $j$ with the lowest draw $a_j$ obtains payoff $1 -a_j^2$, and the other player obtains payoff zero.  The utility function is chosen such that a single player solving the optimization problem is indifferent over all choices $\mu_i$ in expectation.  We show that choosing smaller $\mu_i$ is dominant in the 2-player game.
%We show that choosing smaller $\mu_i$ is dominant.

We supplement our theoretical results with numerical and empirical
ones. First, we test the robustness of our insight on the preference
of bias over variance numerically under distributions other than
normal, and with variations on players' utility functions. Our insight
persists in many of the variations. Second, we consider the same game
but played with learning algorithms on a specific dataset: Players
utilize a ridge regression algorithm on a housing prices dataset,
controlling for the bias-variance tradeoff using a regularization
parameter. With only one player the optimal choice of regularization
parameter may be large (indicating larger bias and lower variance),
but with two players utilities increase as the parameter is lowered
(that is, for lower bias and higher variance).

This paper falls directly into the area described by the fourth bullet
point of the workshop's call for papers, as it studies the effects of
competition between multiple learners.

